Statistical Depth Functions for Ranking Distributions: Definitions, Statistical Learning and Applications

The concept of median/consensus has been widely investigated in order to provide a statistical summary of ranking data, i.e. realizations of a random permutation $\Sigma$ of a finite set, $\{1,\; \ldots,\; n\}$ with $n\geq 1$ say. As it sheds light onto only one aspect of $\Sigma$'s distribution $P$, it may neglect other informative features. It is the purpose of this paper to define analogs of quantiles, ranks and statistical procedures based on such quantities for the analysis of ranking data by means of a metric-based notion of depth function on the symmetric group. Overcoming the absence of vector space structure on $\mathfrak{S}_n$, the latter defines a center-outward ordering of the permutations in the support of $P$ and extends the classic metric-based formulation of consensus ranking (medians corresponding then to the deepest permutations). The axiomatic properties that ranking depths should ideally possess are listed, while computational and generalization issues are studied at length. Beyond the theoretical analysis carried out, the relevance of the novel concepts and methods introduced for a wide variety of statistical tasks are also supported by numerous numerical experiments.

==> application_models.tex <==
\section{Application to popular models}
\label{sec:appli_models}

\subsection{General results for Kendall $\tau$ distance}
\label{subsec:kendall_res}

When the distance $d$ chosen is Kendall $\tau$ distance, we have the following useful result:
\begin{restatable}{proposition}{propdepthkendall}
\label{prop:depth_kendall}
For $d=d_{\tau}$, we have $\vert\vert d_{\tau}\vert\vert_{\infty}=\binom{n}{2}$ and $\forall \; \sigma \in \mathfrak{S}_n$, 

$D_P(\sigma)=\binom{n}{2}-\sum_{i<j} p_{i,j}\mathbb{I}\{\sigma(i)>\sigma(j)\} -\sum_{i<j} (1-p_{i,j})\mathbb{I}\{\sigma(i)<\sigma(j) \}$, 

where $p_{i,j}=\mathbb{P}\{  \Sigma(i)<\Sigma(j)\}$, $1\leq i\neq j\leq n$ are referred to as the pairwise probabilities.
\end{restatable}

This case is computationally attractive, the depth being a $O(n^2)$ expression. In addition, note that the computation of $D_P$ in the Kendall $\tau$ case involves pairwise comparisons solely, which means an alternative statistical framework can be considered, where observation take the form of binary variables $\{\Sigma(\mathbf{i})<\Sigma(\mathbf{j})\}$, $(\mathbf{i},\; \mathbf{j})$ being a random pair in $\{(i,j):\; 1\leq i<j\leq n\}$, independent from $\Sigma$. 

%A crucial property, related to the $p_{i,j}$'s and referred to as \textit{stochastic transitivity} (see \cite{Fishburn73, davidson1959experimental}), is fulfilled by certain ranking distributions, which can be exploited for various statistical tasks (\textit{e.g.} \cite{shah2015stochastically, shah2015simple}).

%\begin{definition}
%\label{def:stoch_trans}
%Let $P$ be a probability distribution on $\mathfrak{S}_n$. It is said to be stochastically transitive iff, for all $(i,j,k)\in \n^3$, we have: $p_{i,j}\geq 1/2 \text{ and } p_{j,k}\geq 1/2 \; \Rightarrow\; p_{i,k}\geq 1/2.$ If, in addition, $p_{i,j}\neq 1/2$ for all $i<j$, one says that $P$ is strictly stochastically transitive.
%\end{definition}
 
%Most popular parametric ranking models, such as the Mallows or the Bradley-Terry-Luce-Plackett model (see \cite{BT52, Luce59, Plackett75}) are stochastically transitive. When then have the following proposition:

\begin{restatable}{proposition}{propkendall}
\label{prop:Kendall}
Suppose that the ranking distribution $P$ is stochastichally transitive (see def. \ref{def:stoch_trans}). The following assertions hold true.
\begin{itemize}
\item[(i)] The largest ranking depth value is $D_P^*= \sum_{i<j}\left\{ \frac{1}{2}+\left\vert p_{i,j}-\frac{1}{2} \right\vert  \right\}$. The deepest rankings relative to $P$ and $d_{\tau}$ are the permutations $\sigma\in\mathfrak{S}_n$ such that: $\forall i<j$ s.t. $p_{i,j}\neq 1/2$, $(\sigma(j)-\sigma(i))\cdot (p_{i,j}-1/2)>0$.
\item[(ii)] The smallest ranking depth value is $D_P^{\star}= \sum_{i<j}\left\{ \frac{1}{2}-\left\vert p_{i,j}-\frac{1}{2} \right\vert  \right\}$. The least deep rankings relative to $P$ and $d_{\tau}$ are the permutations $\sigma\in\mathfrak{S}_n$ such that: $\forall i<j$ s.t. $p_{i,j}\neq 1/2$, $(\sigma(j)-\sigma(i))\cdot (p_{i,j}-1/2)<0$.
\item [(iii)] If, in addition, $P$ is SST, then we have $\partial\mathcal{R}_P(D_P^*)=\{\sigma^*\}$ and $\partial\mathcal{R}_P(D_P^{\star})=\{\sigma^{\star}\}$, where  $\sigma^*(i)=1+\sum_{j\neq i}\mathbb{I}\{p_{i,j}<1/2  \}=n-\sigma^{\star}(i)$ for  $i\in\{1, \; \ldots,\;  n\}$. We also have $D_P^*-D_P(\sigma)=2\sum_{i<j}\vert p_{i,j}-1/2 \vert +D_P(\sigma)-D_P^{\star}
=2\sum_{i<j}\vert p_{i,j}-1/2 \vert \cdot \mathbb{I}\{ (\sigma(j)-\sigma(i))(p_{i,j}-1/2)<0 \}$.
\end{itemize}
\end{restatable}

Refer to section \ref{suppl:proof_kendall} the supplementary for the technical proof and further details.
%When $P$ is strictly stochastically transitive, the mappings $D_P$ and $d_{\tau}(\sigma^*,\; \cdot)$ do not define the same ordering on $\mathfrak{S}_n$ in general, as discussed at length in the Supplementary Material.
%Notice in addition that $\widehat{P}_N$ may be non stochastically transitive and, in such a case, computing a statistical version of $d_{\tau}(\sigma^*,\; \cdot)$ is then far from straightforward (in contrast to the statistical counterpart of $D_P$). Furthermore, when $\widehat{P}_N$ is not stochastically transitive, one cannot rely on Proposition \ref{prop:Kendall}'s formulas to compute an empirical median but a trimming strategy based on the empirical ranking depth can be easily designed for this purpose as described by algo. \ref{algo:trimming}. (see section \ref{suppl:trimming_strat} of the supplementary).

%\begin{algorithm}
%\begin{restatable}{algorithm}{algotrimming}
%\SetKwInOut{Input}{Input}
%\SetKwInOut{Output}{Output}
%\Input{A dataset $S_N=(\sigma_1, ... \sigma_N)$ (its empirical distribution $\hat{P}_N$).}
%\Output{A list of successive medians $L_{med}$ the last one being Kemeny's median $\sigma^*$}

%- Initialize an empty list: $L_{med} = \{\}$\;
%\While{$\hat{P}_N$ is not SST}{
        %\tcc{Say something}
%        - Compute the depth $D_{\hat{P}_N}(\sigma)$ of each ranking $\sigma$ of the dataset $S_N$ \;
%        - Add the deepest ranking $\sigma^{*} = \text{arg} \max_{\sigma} D_{\hat{P}_N}(\sigma)$ to the median list $L_{med}$\;
%        - Remove occurrences of the least deep ranking $\sigma^{\star} = \text{arg} \min_{\sigma} D_{\hat{P}_N}(\sigma)$ in the dataset $S_N$\;
%        - Compute the new empirical distribution $\hat{P}_N$ of the updated dataset $S_N$ \;
%}
%\caption{Trimming strategy}
%\label{algo:trimming}
%\end{restatable}
%\end{algorithm}



\subsection{Mallows distribution and Kendall $\tau$ distance}
\label{subsec:mallow_kendall}

Let us recall some classical results about the Mallows distribution. Taking $d=d_{\tau}$, the Mallows model introduced in \cite{Mallows57} is the unimodal distribution $P_{\theta}$ on $\mathfrak{S}_n$ parametrized by $\theta=(\sigma_0, \phi_0)\in \mathfrak{S}_n\times (0,1]$: $\forall \sigma \in \mathfrak{S}_n$,
$P_{\theta}(\sigma)=(1/Z_0)\exp( d_{\tau}(\sigma_0,\sigma) \log \phi_0)$, where $Z_0=\sum_{\sigma\in \mathfrak{S}_n} \exp(d_{\tau}(\sigma_0,\sigma)\log \phi_0 )$ is a normalization constant.

One may easily show that $Z_0$ is independent from $\sigma_0$ and that $Z_0=\prod_{i=1}^{n-1}\sum_{j=0}^i \phi_0^j$. When $\phi_0<1$, the permutation $\sigma_0$ of reference is the mode of distribution $P_{\theta_0}$, as well as its unique median relative to $d_{\tau}$. Observe in addition that the smallest the parameter $\phi_0$, the spikiest the distribution $P_{\theta_0}$. In contrast, $P_{\theta_0}$ is the uniform distribution on $\mathfrak{S}_n$ when $\phi_0=1$. 

A closed-from expression of the pairwise probabilities $p_{i,j}$ is available (see \textit{e.g.} Theorem 2 in \cite{DBLP:conf/icml/Busa-FeketeHS14}). Setting $h(k,\phi_0)=k/(1-\phi_0^k)$ for $k\geq 1$, one can then show the following: that the ranking depth function relative to $P_{\theta}$ and $d_{\tau}$ is given by:
\begin{restatable}{proposition}{propmallows}
\label{prop:mallows}
If $P = P_{\theta}$ the Mallows distribution and $d=d_{\tau}$ the Kendall $\tau$ distance, then $\forall \sigma\in \mathfrak{S}_n$, $D_{P_{\theta}}(\sigma) = {n \choose 2} - \sum_{\sigma(i)>\sigma(j)} H(\sigma_0(j)-\sigma_0(i),\; \phi_0)$, where $H(k,\phi_0)=h(k+1,\phi_0)-h(k,\phi_0)$ and $H(-k,\phi_0)=1-H(k,\phi_0)$  for $k\geq 1$.
\end{restatable}

